Security Knowledge-Guided Fuzzing of Deep Learning Libraries

Recently, many Deep Learning fuzzers have been proposed for testing of DL libraries. However, they either perform unguided input generation (e.g., not considering the relationship between API arguments when generating inputs) or only support a limited set of corner case test inputs. Furthermore, a substantial number of developer APIs crucial for library development remain untested, as they are typically not well-documented and lack clear usage guidelines. To fill this gap, we propose a novel fuzzer named Orion, which combines guided test input generation and corner case test input generation based on a set of fuzzing rules constructed from historical data that is known to trigger vulnerabilities in the implementation of DL APIs. To extract the fuzzing rules, we first conduct an empirical study regarding the root cause analysis of 376 vulnerabilities in two of the most popular DL libraries, i.e., PyTorch and TensorFlow. We then construct the rules based on the root causes of the historical vulnerabilities. Our evaluation shows that Orion reports 135 vulnerabilities on the latest releases of TensorFlow and PyTorch, 76 of which were confirmed by the library developers. Among the 76 confirmed vulnerabilities, 69 are previously unknown, and 7 have already been fixed. The rest are awaiting further confirmation. Regarding end-user APIs, Orion was able to detect 31.8% and 90% more vulnerabilities on TensorFlow and PyTorch, respectively, compared to the state-of-the-art conventional fuzzer, i.e., DeepRel. When compared to the state-of-the-art LLM-based DL fuzzer, AtlasFuzz, Orion detected 13.63% more vulnerabilities on TensorFlow and 18.42% more vulnerabilities on PyTorch. Regarding developer APIs, Orion stands out by detecting 117% more vulnerabilities on TensorFlow and 100% more vulnerabilities on PyTorch compared to the most relevant fuzzer designed for developer APIs, such as FreeFuzz.

==> sections/implementation.tex <==
\section{Implementation}

==> sections/llm.tex <==
\section{Using LLMs to generate malformed samples}
\label{sec:llm}

\song{ok, if I am a reviewer, I will ask you to compare with and without LLMs in your approach}

Unfortunately, our historical knowledge base lacks a sufficient number of samples for each extracted malformed input generation rule. This scarcity of diverse examples hampers the comprehensiveness of our testing and analysis, potentially leaving some vulnerabilities undiscovered. In response to this limitation, we sought to enhance the sample coverage of malformed inputs by leveraging LLMs. By employing LLMs, we are able to generate a more extensive and diverse set of malformed inputs, effectively augmenting our dataset and providing a broader spectrum of inputs for testing and analysis. With the aid of LLMs, we can explore a wider range of possible input scenarios, enabling us to identify and address vulnerabilities that might have otherwise remained hidden with the limited historical data alone.

The rationale behind employing LLMs for this task lies in their remarkable ability to comprehend context information, which proves instrumental in generating diverse and meaningful samples. To achieve this, we utilize a set of context information as depicted in Figure \ref{fig:llm}. Initially, we transform our rule base into a JSON representation, where multiple records are established, each capturing malformed inputs for various DL data types. Within each record, key-value pairs delineate the rules, along with one real-world sample sourced from open source. Leveraging this context information, we construct a prompt that encapsulates the rules and stores the outcomes in JSON format. Subsequently, utilizing these generated samples, we commence building the fuzzer. 


\begin{figure}[h]
    \centering
    \resizebox{0.3\columnwidth}{!}{{\includegraphics{figures/llmflow.png}}}  
    \caption{The prompt template for generating malicious samples combined with malformed input generation rules.}
    \label{fig:llm}
\end{figure}

==> tables/covered_API.tex <==


% \begin{table*}[t!]
% \caption{Statistics of the number of tested APIs and the value space.
% %Statistics about different sources of APIs. We format the table as Orion/FreeFuzz statistics. 
% % \hung{What is #VS? We have space, maybe spell it out.}
% % \hung{Also I would present the numbers as FreeFuzz/Orion instead, you want to have our approach last.}
% % \hung{For some of these big numbers maybe only present up to 9,999 and then for anything more than that do 10K, for example, 165815 -> 165K.
% % Also, be consistent in the format, 1000 -> 1,000 or never use the comma.} \nima{done}
% }
% \begin{tabular}{lrrrrrrrr}
% \toprule
% \multirow{2}{*}{} & \multicolumn{4}{c}{PyTorch}          & \multicolumn{4}{c}{TensorFlow}       \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% %\midrule
%                   & Doc & Test    & Model & All & Doc & Test    & Model & All \\
%                   \midrule
% \#API             & 427/260 & 176/1,073   & 145/110   & 470/1,075        & 486/338 & 216/2,824   & 269/126   & 688/3,467        \\
% \#Value Space     & 1,259/493 & 3,383/25K & 10K/813   & 15K/253K      & 1,810/526 & 6,879/~20M
%  & 36K/23,419 & 45K/169K     \\
% \bottomrule
% \end{tabular}
% \label{tab:vscovered}
% \end{table*}
